MeGA: Merging Multiple Independently Trained Neural Networks Based on Genetic Algorithm

In this paper, we introduce a novel method for merging the weights of multiple pre-trained neural networks using a genetic algorithm called MeGA. Traditional techniques, such as weight averaging and ensemble methods, often fail to fully harness the capabilities of pre-trained networks. Our approach leverages a genetic algorithm with tournament selection, crossover, and mutation to optimize weight combinations, creating a more effective fusion. This technique allows the merged model to inherit advantageous features from both parent models, resulting in enhanced accuracy and robustness. Through experiments on the CIFAR-10 dataset, we demonstrate that our genetic algorithm-based weight merging method improves test accuracy compared to individual models and conventional methods. This approach provides a scalable solution for integrating multiple pre-trained networks across various deep learning applications. Github is available at: https://github.com/YUNBLAK/MeGA-Merging-Multiple-Independently-Trained-Neural-Networks-Based-on-Genetic-Algorithm

==> contents/results-backup.tex <==
\subsection{Experimental Settings}
% \subsubsection{Dateset 1: CIFAR-10.}
We utilized the CIFAR-10 dataset~\cite{Krizhevsky2009Learning}. The CIFAR-10 training dataset was split into 45,000 training and 5,000 validation sets. The validation set was used during the model validation and merging process. We use CNN models: ResNet~\cite{He2016ResNet}, Xception~\cite{chollet2017xception}, and DenseNet~\cite{huang2017densely} without pre-trained weights and without data augmentation. These models were trained using a batch size of 256 over 50 epochs with the Adam optimizer~\cite{Kingma2014Adam}, using a learning rate of 0.01.


% \subsubsection{Other datasets}
% The PatchCamelyon dataset~\cite{patch-1} is a benchmark dataset for histopathologic cancer detection. It contains image patches extracted from whole-slide images of lymph node sections. The dataset~\cite{path-2} we used was a slightly modified version of the original PatchCamelyon dataset~\cite{patch-1}. We used the PatchCamelyon dataset, which consists of 30,000 training images, 10,000 test images, and 10,000 validation images. Each image patch is converted to 32x32 pixels. ResNets (56, 110, 156) were trained using a batch size of 256 over 20 epochs with the Adam optimizer~\cite{Kingma2014Adam} and a learning rate of 0.01. No data augmentation was applied during training.


% \setlength{\tabcolsep}{2pt}
% \begin{table}[htbp]
% \centering
% \caption{Performance Comparison of Individual and MeGA-Merged CNN Models based on MeGA with CIFAR-10 Dataset}
% \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{@{}l|lllcc@{}}
% \toprule
% \toprule
% Dataset& Model (\# of Params.) & & Baseline & Baseline Acc. & Final Test Acc.  \\
% \# of Classes && & (Random Seed) & (Single Model) & (Merged Model)  \\

% \toprule
%  &\multirow{2}{*}{ResNet 56 (0.86M)~\cite{He2016ResNet}} & \ \ \ & Model 1 (56) & 0.809 &  \multirow{2}{*}{0.822} \\
%                                     &&& Model 2 (57) & 0.793 &  \\
%                   \cline{2-6}                 
% &\multirow{2}{*}{ResNet 110 (1.78M)~\cite{He2016ResNet}} && Model 1 (56) & 0.801 &  \multirow{2}{*}{0.816} \\
%                                      &&& Model 2 (57) & 0.814 &  \\
%                    \cline{2-6}                
% &\multirow{2}{*}{ResNet 152 (3.51M)~\cite{He2016ResNet}} && Model 1 (56) & 0.783 &  \multirow{2}{*}{0.819} \\
%                                     CIFAR-10~\cite{Krizhevsky2009Learning}  &&& Model 2 (57) & 0.781 &  \\
%                   \cline{2-6}                
% 10 &\multirow{2}{*}{Xception (22.96M)~\cite{He2016ResNet}} && Model 1 (56) & 0.716 &  \multirow{2}{*}{0.754} \\
%                                     &&& Model 2 (57) & 0.730 &  \\
%                    \cline{2-6}                 
% &\multirow{2}{*}{DenseNet 121 (7.04M)~\cite{He2016ResNet}} && Model 1 (56) & 0.719 &  \multirow{2}{*}{0.742} \\
%                                     &&& Model 2 (57) & 0.728 &  \\
%                    \cline{2-6}                
% &\multirow{2}{*}{DenseNet 169 (12.65M)~\cite{He2016ResNet}} && Model 1 (56) & 0.735 &  \multirow{2}{*}{0.753} \\
%                                     &&& Model 2 (57) & 0.731 &  \\
% %                     \midrule                
% % \multirow{2}{*}{EfficientNetB1(12.65M)~\cite{He2016ResNet}} & EfficientNetB1 Model 1 (56) & 0.735 &  0.753 \\
% %                                     & EfficientNetB1 Model 2 (57) & 0.731 &  0.753 \\                                    
% % \midrule
% % Mean 
% % & &  & 0.0002 & 1.5x \\
% \bottomrule
% \bottomrule
% \end{tabular}
% \label{tab:cnn}
% \end{adjustbox}
% \end{table}

% \subsubsection{Merge process.}
Each model followed the same architecture and hyperparameters to ensure consistency and a fair comparison. After training, we applied our MeGA approach to merge the weights of these models into a single set of weights. The performance of the merged model was then evaluated and compared against the individual models. For all experiments, we used the following MeGA hyperparameters: a population size of 20, 20 generations, 4 parents per generation, and a mutation rate of 0.02.



\subsection{CIFAR-10 Results}
The results of the image classification experiments on the CIFAR-10 dataset~\cite{Krizhevsky2009Learning} demonstrate the effectiveness of our MeGA.

\setlength{\tabcolsep}{2pt}
\begin{table}[htbp]
\centering
\caption{Performance Comparison of Individual and MeGA-Merged CNN Models based on MeGA with CIFAR-10 Dataset}
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{@{}l|lllcc@{}}
\toprule
\toprule
Dataset & Model (\# of Params.) & & Baseline & Baseline Acc. & Final Test Acc.  \\
& & & (Random Seed) & (Single Model) & (Merged Model)  \\

\toprule
 & \multirow{2}{*}{ResNet 56 (0.86M)~\cite{He2016ResNet}} & \ \ \ & Model 1 (56) & 0.920 &  \multirow{2}{*}{0.945} \\
                                    &&& Model 2 (57) & 0.942 &  \\
                  \cline{2-6}               
SVHN~\cite{He2016ResNet} &\multirow{2}{*}{ResNet 110 (1.78M)~\cite{He2016ResNet}} && Model 1 (56) & 0.801 &  \multirow{2}{*}{0.816} \\
                                     (10) &&& Model 2 (57) & 0.814 &  \\
                   \cline{2-6}                  
&\multirow{2}{*}{ResNet 152 (3.51M)~\cite{He2016ResNet}} && Model 1 (56) & 0.783 &  \multirow{2}{*}{0.819} \\
                                    &&& Model 2 (57) & 0.781 &  \\

\midrule  

 & \multirow{2}{*}{ResNet 56 (0.86M)~\cite{He2016ResNet}} & \ \ \ & Model 1 (56) & 0.830 &  \multirow{2}{*}{0.862} \\
                                    &&& Model 2 (57) & 0.860 &  \\
                  \cline{2-6}               
Caltech-101~\cite{He2016ResNet} &\multirow{2}{*}{ResNet 110 (1.78M)~\cite{He2016ResNet}} && Model 1 (56) & 0.801 &  \multirow{2}{*}{0.816} \\
                                    (10) &&& Model 2 (57) & 0.814 &  \\
                   \cline{2-6}                  
&\multirow{2}{*}{ResNet 152 (3.51M)~\cite{He2016ResNet}} && Model 1 (56) & 0.783 &  \multirow{2}{*}{0.819} \\
                                    &&& Model 2 (57) & 0.781 &  \\

\midrule  

 & \multirow{2}{*}{ResNet 56 (0.86M)~\cite{He2016ResNet}} & \ \ \ & Model 1 (56) & 0.830 &  \multirow{2}{*}{0.862} \\
                                    &&& Model 2 (57) & 0.860 &  \\
                  \cline{2-6}               
SVHN~\cite{He2016ResNet} &\multirow{2}{*}{ResNet 110 (1.78M)~\cite{He2016ResNet}} && Model 1 (56) & 0.801 &  \multirow{2}{*}{0.816} \\
                                    (10) &&& Model 2 (57) & 0.814 &  \\
                   \cline{2-6}                  
&\multirow{2}{*}{ResNet 152 (3.51M)~\cite{He2016ResNet}} && Model 1 (56) & 0.783 &  \multirow{2}{*}{0.819} \\
                                    &&& Model 2 (57) & 0.781 &  \\

%                     \midrule                
% \multirow{2}{*}{EfficientNetB1(12.65M)~\cite{He2016ResNet}} & EfficientNetB1 Model 1 (56) & 0.735 &  0.753 \\
%                                     & EfficientNetB1 Model 2 (57) & 0.731 &  0.753 \\                                    
% \midrule
% Mean 
% & &  & 0.0002 & 1.5x \\
\bottomrule
\bottomrule
\end{tabular}
\label{tab:tumor}
\end{adjustbox}
\end{table}

The MeGA approach led to significant improvements in test accuracies across various models as shown in the Table~\ref{tab:cnn}. For example, the ResNet 56 model's accuracy improved from 0.801 to 0.822, and the ResNet 110 model reached 0.824. 

\begin{figure}
\centering
\includegraphics[width=1.0\columnwidth]{figures/generation.png}
\caption{MeGA Fitness Progression (Test Accuracy) for ResNet-56 and DenseNet 121 models over 20 generations.}
\label{fig:MeGA_fitness_progression}
\end{figure}

The Xception model's accuracy increased from 0.723 to 0.754, demonstrating the effectiveness of MeGA in optimizing complex architectures. Similarly, the DenseNet 121 model's accuracy rose from 0.724 to 0.742, and the DenseNet 169 model improved from 0.733 to 0.753. Overall, the MeGA approach consistently outperformed individual models, highlighting its potential for enhancing neural network performance through genetic algorithm-based weight merging.

Figure~\ref{fig:MeGA_fitness_progression} shows the progression of the best fitness values over 20 generations for the ResNet-56 and DenseNet 121 models. For the ResNet-56 model, the best fitness improved steadily from 0.8042 in the first generation to 0.8224 in the twentieth generation. Similarly, the DenseNet 121 model saw an improvement in best fitness from 0.7290 to 0.7427 over the same period. These plots illustrate the genetic algorithm's capability to effectively navigate the weight space and optimize combinations to enhance model performance.



% The improvements in fitness values were reflected in the test accuracies of the models. The ResNet models of varying depths (56, 110, and 152 layers) showed improvements in test accuracy after merging the weights using the MeGA approach. For instance, the ResNet 56 model's test accuracy improved from an average of 0.801 to 0.822. The ResNet 110 model, which has 1.78 million parameters, demonstrated a final test accuracy of 0.824 after merging, indicating that the MeGA approach effectively leveraged the strengths of the individual models.

% Similarly, the Xception model, which uses depthwise separable convolutions, saw an increase in test accuracy from an average of 0.723 to 0.754 after the MeGA-based weight merging. This improvement highlights the MeGA approach's ability to optimize and combine complex model architectures effectively.

% The DenseNet models (121 and 169 layers) also benefited from the MeGA approach, with improvements in test accuracy. The DenseNet 121 model's accuracy increased from an average of 0.724 to 0.742, while the DenseNet 169 model's accuracy increased from 0.733 to 0.753.

% Overall, the MeGA approach consistently outperformed the individual models in terms of test accuracy. The merged model's performance was significantly better than that of any single model, demonstrating the potential of the MeGA approach in optimizing and combining neural network weights to achieve superior performance. This suggests that the genetic algorithm-based weight merging technique is a viable and efficient method for enhancing the performance of neural networks by integrating multiple pre-trained models.


% \subsection{Other Datasets}

% The improvements in fitness values were reflected in the test accuracies of the models. The ResNet models of varying depths (56, 110, and 152 layers) showed improvements in test accuracy after merging the weights using the MeGA approach. For instance, the ResNet 56 model's test accuracy improved from an average of 0.801 to 0.822. The ResNet 110 model, which has 1.78 million parameters, demonstrated a final test accuracy of 0.824 after merging, indicating that the MeGA approach effectively leveraged the strengths of the individual models.

% \setlength{\tabcolsep}{2pt}
% \begin{table}[htbp]
% \centering
% \caption{Performance Comparison of Individual and MeGA-Merged CNN Models based on MeGA with CIFAR-10 Dataset}
% \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{@{}l|lllcc@{}}
% \toprule
% \toprule
% Dataset & Model (\# of Params.) & & Baseline & Baseline Acc. & Final Test Acc.  \\
% & & & (Random Seed) & (Single Model) & (Merged Model)  \\

% \toprule
%  & \multirow{2}{*}{ResNet 56 (0.86M)~\cite{He2016ResNet}} & \ \ \ & Model 1 (56) & 0.920 &  \multirow{2}{*}{0.945} \\
%                                     &&& Model 2 (57) & 0.942 &  \\
%                   \cline{2-6}               
% SVHN~\cite{He2016ResNet} &\multirow{2}{*}{ResNet 110 (1.78M)~\cite{He2016ResNet}} && Model 1 (56) & 0.801 &  \multirow{2}{*}{0.816} \\
%                                      (10) &&& Model 2 (57) & 0.814 &  \\
%                    \cline{2-6}                  
% &\multirow{2}{*}{ResNet 152 (3.51M)~\cite{He2016ResNet}} && Model 1 (56) & 0.783 &  \multirow{2}{*}{0.819} \\
%                                     &&& Model 2 (57) & 0.781 &  \\

% \midrule  

%  & \multirow{2}{*}{ResNet 56 (0.86M)~\cite{He2016ResNet}} & \ \ \ & Model 1 (56) & 0.830 &  \multirow{2}{*}{0.862} \\
%                                     &&& Model 2 (57) & 0.860 &  \\
%                   \cline{2-6}               
% Caltech-101~\cite{He2016ResNet} &\multirow{2}{*}{ResNet 110 (1.78M)~\cite{He2016ResNet}} && Model 1 (56) & 0.801 &  \multirow{2}{*}{0.816} \\
%                                     (10) &&& Model 2 (57) & 0.814 &  \\
%                    \cline{2-6}                  
% &\multirow{2}{*}{ResNet 152 (3.51M)~\cite{He2016ResNet}} && Model 1 (56) & 0.783 &  \multirow{2}{*}{0.819} \\
%                                     &&& Model 2 (57) & 0.781 &  \\

% \midrule  

%  & \multirow{2}{*}{ResNet 56 (0.86M)~\cite{He2016ResNet}} & \ \ \ & Model 1 (56) & 0.830 &  \multirow{2}{*}{0.862} \\
%                                     &&& Model 2 (57) & 0.860 &  \\
%                   \cline{2-6}               
% SVHN~\cite{He2016ResNet} &\multirow{2}{*}{ResNet 110 (1.78M)~\cite{He2016ResNet}} && Model 1 (56) & 0.801 &  \multirow{2}{*}{0.816} \\
%                                     (10) &&& Model 2 (57) & 0.814 &  \\
%                    \cline{2-6}                  
% &\multirow{2}{*}{ResNet 152 (3.51M)~\cite{He2016ResNet}} && Model 1 (56) & 0.783 &  \multirow{2}{*}{0.819} \\
%                                     &&& Model 2 (57) & 0.781 &  \\

% %                     \midrule                
% % \multirow{2}{*}{EfficientNetB1(12.65M)~\cite{He2016ResNet}} & EfficientNetB1 Model 1 (56) & 0.735 &  0.753 \\
% %                                     & EfficientNetB1 Model 2 (57) & 0.731 &  0.753 \\                                    
% % \midrule
% % Mean 
% % & &  & 0.0002 & 1.5x \\
% \bottomrule
% \bottomrule
% \end{tabular}
% \label{tab:tumor}
% \end{adjustbox}
% \end{table}

% Similarly, the Xception model, which uses depthwise separable convolutions, saw an increase in test accuracy from an average of 0.723 to 0.754 after the MeGA-based weight merging. This improvement highlights the MeGA approach's ability to optimize and combine complex model architectures effectively.

% The DenseNet models (121 and 169 layers) also benefited from the MeGA approach, with improvements in test accuracy. The DenseNet 121 model's accuracy increased from an average of 0.724 to 0.742, while the DenseNet 169 model's accuracy increased from 0.733 to 0.753.

\begin{figure}
\centering
\includegraphics[width=1.0\columnwidth]{figures/GANN2.png}
\caption{Hierarchical merging process of eight models into a single final model.}
\label{fig:merge}
\end{figure}

\subsection{Extended Experiments for Multi-Models}
In this section, we illustrate the application of our genetic algorithm-based weight merging method to combine multiple neural network models as depicted in Figure~\ref{fig:merge}.



\setlength{\tabcolsep}{3pt}
\begin{table}[htbp]

\centering
\caption{Performance Comparison of 8 Individual and Merged ResNet Models based on MeGA with CIFAR-10 Dataset}
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{@{}l|lllcc@{}}
\toprule
\toprule
Dataset &Model (\# of Params) & & Baseline. & Baseline Test Acc. & Final Test Acc.  \\
\# of classes &&& (Random Seed) & (Single Model) & (Merged Model)\\
\midrule
&\multirow{8}{*}{ResNet 56 (0.86M)~\cite{He2016ResNet}} & & Model 1 (44) & 0.804 & \multirow{8}{*}{0.822} \\
&& & Model 2 (45) & 0.747 & \\
&& & Model 3 (46) & 0.788 & \\
&& & Model 4 (47) & 0.774 & \\
&& & Model 5 (48) & 0.806 & \\
&& & Model 6 (49) & 0.786 & \\
&& & Model 7 (50) & 0.749 & \\
&& & Model 8 (51) & 0.787 & \\
\cline{2-6}   
&\multirow{8}{*}{ResNet 110 (1.78M)~\cite{He2016ResNet}} & & Model 1 (44) & 0.782 & \multirow{8}{*}{0.824} \\
&& & Model 2 (45) & 0.814 & \\
&& & Model 3 (46) & 0.744 & \\
CIFAR-10~\cite{Krizhevsky2009Learning}&& & Model 4 (47) & 0.800 & \\
(10)&& & Model 5 (48) & 0.801 & \\
&& & Model 6 (49) & 0.787 & \\
&& & Model 7 (50) & 0.781 & \\
&& & Model 8 (51) & 0.758 & \\
\cline{2-6}   
&\multirow{8}{*}{ResNet 152 (3.51M)~\cite{He2016ResNet}} & & Model 1 (44) & 0.775 & \multirow{8}{*}{0.815} \\
&& & Model 2 (45) & 0.783 & \\
&& & Model 3 (46) & 0.781 & \\
&& & Model 4 (47) & 0.747 & \\
&& & Model 5 (48) & 0.771 & \\
&& & Model 6 (49) & 0.767 & \\
&& & Model 7 (50) & 0.772 & \\
&& & Model 8 (51) & 0.797 & \\
\bottomrule
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:cnn}
\end{table}

The hierarchical merging process starts by training eight models on the CIFAR-10 dataset~\cite{He2016ResNet, Krizhevsky2009Learning}. These models are paired and merged using a genetic algorithm, resulting in four intermediate models. These intermediate models are further merged into two higher-level models, which are finally merged into a single, robust model. This process ensures the final model combines the strengths of all eight original models. The results in Table~\ref{tab:cnn} demonstrate the effectiveness of our genetic algorithm-based weight merging method. For ResNet 56 models, baseline test accuracies ranged from 0.747 to 0.806, improving to 0.822 after merging. ResNet 110 models had baseline accuracies between 0.744 and 0.814, with the merged model achieving 0.824. For ResNet 152 models, baseline accuracies ranged from 0.747 to 0.783, and the merged model reached 0.815. Despite the larger complexity of ResNet 152, our method effectively enhanced model performance.

These results highlight the potential of our approach to enhance neural network performance. The consistent improvement in test accuracy across different architectures (ResNet 56, ResNet 110, and ResNet 152) demonstrates the versatility and scalability of our method. The hierarchical merging process ensures the final model benefits from the strengths of individual models.


